Can Increasing the Hit Ratio Hurt Cache Throughput? (Long Version)

Software caches are an intrinsic component of almost every computer system. Consequently, caching algorithms, particularly eviction policies, are the topic of many papers. Almost all these prior papers evaluate the caching algorithm based on its hit ratio, namely the fraction of requests that are found in the cache, as opposed to disk. The hit ratio is viewed as a proxy for traditional performance metrics like system throughput or response time. Intuitively it makes sense that higher hit ratio should lead to higher throughput (and lower response time), since more requests are found in the cache (low access time) as opposed to the disk (high access time). This paper challenges this intuition. We show that increasing the hit ratio can actually hurt the throughput (and response time) for many caching algorithms. Our investigation follows a three-pronged approach involving (i) queueing modeling and analysis, (ii) implementation and measurement, and (iii) simulation to validate the accuracy of the queueing model. We also show that the phenomenon of throughput decreasing at higher hit ratios is likely to be more pronounced in future systems, where the trend is towards faster disks and higher numbers of cores per CPU.

==> ancient/1.intro_old.tex <==

\section{Introduction}

* introduce cache and cache replacement 
    * eviction 
        * The popularity of LRU-based caches 
        * FIFO 
        * more complex 

    * admission 
    
* The importance of scalability 
    * justify why high MPL 
    * open vs closed system

* the metrics used to evaluate caching policies
    * common metrics: throughput and latency 
    * hit ratio as a proxy for obtaining better throughput and latency 
        * other reasons for favoring a high hit ratio: load shedding, wear and tear
        
* the claim: despite intuition (high hit ratio -> increased throughput), we will show this may not hold
    * results: we show for LRU and FIFO 
    * table shows the summary of result (whether a high hit ratio helps)
    
* methodology in three folds 
    * models of the caches and queuing theory to show what should happen, give a rough guide of the model, asymptote
    * simulation of the queuing model to estimate the full spectrum
    * extensive implementations to validate the results 
    * all agree 


takeaway
* how miss ratio and latency/throughput can diverge 
* system-design lessons: 
    * implications for new cache eviction algorithm design 
        * more queues relieve the problem
        * fifo queues are better
    * run an LRU cache with a lower hit ratio (NHC)
    *     









* talk about queue theory basics
    * talk about the model of LRU queues
    * open vs closed system

* talk about the result 
    * the metrics do not align with each other
    * explain why briefly
    * the implication of the results 



==> ancient/4.queueingAnalysis.tex <==

\section{Queueing-theoretic analysis}
\label{s:analysis}

The goal is not response time as a function of $N$.

I think we should limit the goals here:
\begin{enumerate}
\item Specify a few settings of parameters.
\item For each parameter setting and each policy, what is the point at which increasing hit ratio stops helping?
\item Take-aways about policies.
  \end{enumerate}



==> ancient/mystyleprob2.tex <==
%\usepackage{graphics} % for pdf, bitmapped graphics files

%\usepackage[pdftex]{graphicx}

%\setlength{\textheight}{8.5in}
%\setlength{\oddsidemargin}{0.2in}
%\setlength{\evensidemargin}{0.2in}
%\setlength{\topmargin}{-0.3in}


\setlength{\parindent}{0.6in}
\setlength{\unitlength}{1cm}
\setlength{\textwidth}{6.4in}
\setlength{\parskip}{0.0in}
%\setlength{\parskip}{0.14in}

\newcommand{\pfhead}{\noindent {\bf Proof:}\ }
\newcommand{\dpfhead}[1]{\noindent {\bf Proof of Theorem~\ref{#1}:}\ }

\def\squarebox#1{\hbox to #1{\hfill\vbox to #1{\vfill}}}
\newcommand{\qedbox}{\vbox{\hrule\hbox{\vrule\squarebox{.667em}\vrule}\hrule}}
% \newcommand{\qed}{\nopagebreak\mbox{}\hfill\qedbox\bigskip}
\newcommand{\ibits}{\{0,1\}^\infty}
\newcommand{\Nat}{\mathcal{N}}
\newcommand{\itbits}{\{011,110\}^\infty}
\newcommand{\srpt}{\mathtt{SRPT\text{-}1}}
\newcommand{\srptk}{\mathtt{SRPT\text{-}k}}
\newcommand{\rwork}{\mathtt{RWork}}
\newcommand{\work}{\mathtt{Work}}
%\newcommand{\psfig}[1]{\epsfig{#1}}


% \newcommand{\state}{\pi_{(c^{(1)}, c^{(2)}, \ldots, c^{(n)})}}
\newcommand{\substate}[2]{\left(c^{(1)}_{#1}, c^{(2)}_{#1}, \ldots, c^{(#2)}_{#1}\right)}
\newcommand{\comb}[2]{\left( \begin{array}{c} #1 \\ #2 \end{array} \right)}

\newcommand{\markend}{\hfill \rule{0.25cm}{0.25cm}}
\newcommand{\thickline}{\noindent \rule{16.5cm}{0.08cm}}




%-- enclose something in parens, brackets, or braces
\newcommand{\parens}[1]{{\left( #1 \right)}}
\newcommand{\bracks}[1]{{\left[ #1 \right]}}
\newcommand{\braces}[1]{{\left\{ #1 \right\}}}



%--random variables:  random var X is  \rv{X}
%\newcommand{\rv}[1]{\ensuremath{\mathbf{#1}}}

%--variance: variance of X is \var{\rv{X}}
\newcommand{\Var}[1]{{\mbox{\bf Var}\parens{#1}}}
\newcommand{\std}[1]{{\mbox{\bf std}\parens{#1}}}
\newcommand{\Skew}[1]{{\mbox{\bf Skew}\parens{#1}}}
\newcommand{\cov}[1]{{\mbox{cov}\parens{#1}}}
\newcommand{\Exp}{\mbox{Exp}}
\newcommand{\argmax}{\mbox{argmax}}
\newcommand{\Normal}{\mbox{Normal}}
\newcommand{\Bernoulli}{\mbox{Bernoulli}}
\newcommand{\Binomial}{\mbox{Binomial}}
\newcommand{\Pareto}{\mbox{Pareto}}
\newcommand{\BoundedPareto}{\mbox{BoundedPareto}}
\newcommand{\Poisson}{\mbox{Poisson}}
\newcommand{\Uniform}{\mbox{Uniform}}
\newcommand{\Erlang}{\mbox{Erlang}}
\newcommand{\Geometric}{\mbox{Geometric}}
\color{blue}
\newcommand{\Cov}[2]{{\mbox{\bf Cov}\parens{#1,#2}}}
\color{black}

% This is the gizmo.  Put it into mystyle
\newcommand{\MatBorderStyle}[1]{{\textcolor{Gray}{#1}}}
\newcommand{\MatBorderStyletiny}[1]{{\mbox{\tiny{$\MatBorderStyle{#1}$}}}}
\newcommand{\MatBorderStylescript}[1]{{\mbox{\scriptsize{$\MatBorderStyle{#1}$}}}}
\newcommand{\MatBorderStylefoot}[1]{{\mbox{\footnotesize{$\MatBorderStyle{#1}$}}}}
\newcommand{\mathtiny}[1]{{\mbox{\tiny{$#1$}}}}
\newcommand{\mathscript}[1]{{\mbox{\tiny{$#1$}}}}
\newcommand{\mathfoot}[1]{{\mbox{\tiny{$#1$}}}}
\newcommand{\zerovec}{\vec{0}}
%\newcommand{\onevec}{\vec{e}}
\newcommand{\onevec}{\vec{1}}

\makeatletter
\def\bordermatrix{\@bordermatrix@i*}%
\def\@bordermatrix@i*{\@ifnextchar[{%
  \@bordermatrix@ii}{\@bordermatrix@ii[()][\quad]}
}
\def\@bordermatrix@ii[#1][#2]#3{%
  \begingroup
	%\offinterlineskip
    \m@th\@tempdima4.75\p@\setbox\z@\vbox{%
      \def\cr{\crcr\noalign{\kern 2\p@\global\let\cr\endline}}%
      \ialign {$##$\hfil\kern 2\p@\kern\@tempdima & \thinspace %
      \hfil $##$\hfil && \@#2\hfil $##$\hfil\crcr\omit\strut %
      \hfil\crcr\noalign{\kern -\baselineskip}#3\crcr\omit %
      \strut\cr}}%
    \setbox\tw@\vbox{\unvcopy\z@\global\setbox\@ne\lastbox}%
    \setbox\tw@\hbox{\unhbox\@ne\unskip\global\setbox\@ne\lastbox}%
    \setbox\tw@\hbox{%
      $\kern\wd\@ne\kern -\@tempdima\left\@firstoftwo#1\kern -\wd\@ne\global\setbox\@ne\vbox{\box\@ne\kern 2\p@}%
      \vcenter{\kern -\ht\@ne\unvbox\z@\kern-\baselineskip}\right] $%
    }\null \;\vbox{\kern\ht\@ne\box\tw@}%
  \endgroup
}
\makeatother
% this ends the gizmo


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  math.sty %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\up=\uparrow
\let\down=\downarrow
%\let\inf=\infty
% Ziv: redefining \empty conflicts with enumitem
% \let\empty=\emptyset
\def\P#1{\mathrm{\bf P}\left\{#1\right\}}	%Probability:  P{...}
\def\E#1{\mathrm{\bf E}\left[#1\right]}		%Expectation:  E{...}
\def\V#1{\mathrm{\bf Var}\left\{#1\right\}}	%Variance:   Var{...}
\def\Caption#1{\caption{\emph {#1}}} % Change to single spacing

\def\degrees{^\circ}
\let\check\surd
\def\code#1{\langle #1 \rangle}
\def\Sum{\displaystyle\sum}
\def\Prod{\displaystyle\prod}
\def\Int{\displaystyle\int}
\def\T{\mbox{\bf T}}  %true
\def\F{\mbox{\bf F}}  %false
\let\bar=\overline
\let\reducesto=\propto
\def\half{\mbox{$1 \over 2$}}
\def\th{^{\rm th}}
\def\st{\hbox{\it\ s.t.\ }}
\def\ow{\hbox{\it\ o.w.\ }}
% \def\gets{\leftarrow}
% \def\iff{\Leftrightarrow}
\let\by=\times
\def\implies{\ \Rightarrow\ }
\def\eqd{\ \stackrel{\rm d}{=}\ }
\def\eqdef{\ \stackrel{\rm def}{=}\ }
\def\geqas{\ \underset{\rm as}{\geq}}
\def\gas{\ \underset{\rm as}{>}}
\def\leqas{\ \underset{\rm as}{\leq}}
\def\las{\ \underset{\rm as}{<}}
\def\geqst{\ \underset{\rm st}{\geq}}
\def\gst{\ \underset{\rm st}{>}}
\def\leqst{\ \underset{\rm st}{\leq}}
\def\lst{\ \underset{\rm st}{<}}
\def\geqhr{\ \underset{\rm hr}{\geq}}
\def\ghr{\ \underset{\rm hr}{>}}
\def\leqhr{\ \underset{\rm hr}{\leq}}
\def\lhr{\ \underset{\rm hr}{<}}
\def\geqlr{\ \underset{\rm lr}{\geq}}
\def\glr{\ \underset{\rm lr}{>}}
\def\leqlr{\ \underset{\rm lr}{\leq}}
\def\llr{\ \underset{\rm lr}{<}}
\def\geqcx{\ \underset{\rm cx}{\geq}}
\def\gcx{\ \underset{\rm cx}{>}}
\def\leqcx{\ \underset{\rm cx}{\leq}}
\def\lcx{\ \underset{\rm cx}{<}}
\def\geqicx{\ \underset{\rm icx}{\geq}}
\def\gicx{\ \underset{\rm icx}{>}}
\def\leqicx{\ \underset{\rm icx}{\leq}}
\def\licx{\ \underset{\rm icx}{<}}
\def\leapprox{\ \stackrel{<}{\sim}\ }
\def\geapprox{\ \stackrel{>}{\sim}\ }
% \def\=}{\eqdef
\let\xor=\oplus
\let\Or=\vee
\let\And=\wedge
\def\OR{\displaystyle\bigvee}
\def\AND{\displaystyle\bigwedge}
\def\given{\ |\ }
\let\union=\cup
\let\Union=\bigcup
\let\intersect=\cap
\let\Intersect=\bigcap
\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}

\def\QuadSpace{\vspace{0.25\baselineskip}}
\def\HalfSpace{\vspace{0.5\baselineskip}}
\def\FullSpace{\vspace{1.0\baselineskip}}
\def\EndProof{ \quad \vrule width 1ex height 1ex depth 0pt \newline }

\newtheorem{theorem}{Theorem}

%%\renewcommand{\labelenumi}{\thechapter.\arabic{enumi}}
%%\renewcommand{\theenumi}{\thechapter.\arabic{enumi}}
%\newcounter{Theoremcount}[chapter]
%
%\newtheorem{theorem}[Theoremcount]{Theorem}
%\newtheorem{observation}{Observation}
%\newtheorem{example}{Example}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}[Theoremcount]{Definition}
%\newtheorem{claim}{Claim}
%\newtheorem{fact}[claim]{Fact}
%\newtheorem{fact}{Fact}
% \newenvironment{proof}{\QuadSpace\par\noindent{\bf Proof}:}{\EndProof\HalfSpace}
\newenvironment{Proof}{\QuadSpace\par\noindent{\bf Proof}:}{\HalfSpace}

\newenvironment{Figure}{\begin{figure}[hbtp]}{\end{figure}}
\newenvironment{Table}{\begin{table}[hbtp]}{\end{table}}

%\makeatletter
%\newtheorem{rep@theorem}{\rep@title}
%\newcommand{\newreptheorem}[2]{%
%\newenvironment{rep#1}[1]{%
% \def\rep@title{#2 \ref{##1}}%
% \begin{rep@theorem}}%
% {\end{rep@theorem}}}
%\makeatother
%
%\newreptheorem{theorem}{Theorem}
%\newreptheorem{lemma}{Lemma}

\def\ep{\epsilon}
\def\sgn{\mathop{\rm sgn}}


==> ancient/old.tex <==

******************************************************* \newline
************* OLD STUFF  ****************************** \newline
******************************************************* \newline

\section{Modeling an LRU Cache}

We have requests which are trying to get data.

Our system has $72$ cores.  This limits the number of requests that can be in the system simultaneously to $72$, since each request is assigned to one core.  

The disk has enough concurrency that all requests that go to disk can access the disk simultaneously.   A {\bf Disk Access} requires $100\mu s$ on average.  

Additionally, there is a shared cache.  The {\bf Cache Access} time is much faster access time than the Disk Access.  Specifically, Cache Access takes on average $0.65\mu s$.  The cache can be accessed simultaneously by all 72 cores.  To search the cache quickly, we use a hash table, which returns a list of items that must be traversed.

To implement the {\bf LRU policy} we additionally store {\em all} cached items into a single {\bf global linked list}, 
where the least-recently-used item is the ``tail'' item of the list and is the one dropped, while the most-recently-used item is at ``head'' of the list.

Every request first goes to the cache to look for the data (let’s call the data item $d$).   Either the request finds $d$ in the cache (called a ``hit”), or it doesn’t (called a ``miss”).  

If the request is a hit, then two things need to happen:
\begin{enumerate}
\item The item, $d$, needs to be unlinked from its position in the global linked list (front and back pointers removed).  This is called the {\bf Delink operation}, and it takes on average $0.9\mu s$.
\item The item, $d$, needs to be attached to the Head of the global linked list.  This is called the {\bf Cache Head update}, and it takes on average $0.245\mu s$.
\end{enumerate}

If the request is a miss, then three things need to happen:
\begin{enumerate}
\item The item, $d$, needs to be found on disk.   Recall this {\bf Disk Access} takes $100\mu s$ on average.
\item The least-recently-used item (the one at the tail of the global linked cache list) needs to be removed.  We call this the {\bf Cache Tail update}, and it takes $0.3\mu s.$
\item Item $d$ needs to be attached to the Head of the global linked list.  This is the {\bf Cache Head update} that we mentioned earlier.
\end{enumerate}

The probability of a hit is denoted by $p_{hit}$ and the probability of a miss is $p_{miss}$, where $$p_{hit} + p_{miss} = 1. $$

Given all the above, we can model the LRU Caching system via the queueing model shown in Figure~\ref{fig:LRUcache}.  We will see that this queueing network in Figure~\ref{fig:LRUcache} is an excellent model of our real system.   We will next show a queueing analysis of this model using Operational Laws.  Later we will also simulate the queueing network and compare that with implementation results, showing an excellent fit. 

\begin{figure}[ht]
\centerline{\psfig{file=figs/LRUcache.eps,height=2.5in}}
\caption{Queueing model of LRU cache.}
\label{fig:LRUcache}
\end{figure}

\section{Queueing-theoretic analysis of the LRU queueing model}

We now use Operation Laws and ``what-if'' analysis to analyze the queueing model of Figure~\ref{fig:LRUcache}, following the approach of \cite[Chapters 6,7]{PerformanceModeling13}.

The network is a closed-batch network, with multiprogramming limit $N = \mbox{MPL} = 72$ and mean think time of

$$\E{Z} = \E{Z_{cache}} + p_{miss} \cdot \E{Z_{disk}} = 0.65 + 100 p_{miss} . $$

  The device demands are as follows:

  \begin{eqnarray*}
D_{delink} & = & p_{hit} \cdot 0.9 \\
D_{tail} & = & p_{miss} \cdot 0.3 \\
D_{head} & = & 0.245 
    \end{eqnarray*}

  For every reasonable value of $p_{hit}$ (anything greater than about 30\%), $D_{delink}$ is the highest of the device demands.  Hence it is reasonable to assume that the bottleneck device demand is
  $$D_{max} = D_{delink} = p_{hit} \cdot 0.9. $$

  The goal of increasing throughput, $X$, is to decrease the demand on the bottleneck device, and this points to {\em decreasing} $p_{hit}$, which is certainly counter-intuitive.

  However the problem is not quite that simple, because throughput is actually bounded by $2$ terms, the first of which is the asymptote for low $N$ and the second of which is the asymptote for high $N$.  To understand whether $N = 72$ is high or low requires evaluating $N^*$.  We now write out all these details:

  We first define the {\em total demand}, $D$:
\begin{eqnarray*}
  D & = &  D_{delink} + D_{tail} + D_{head}  \\
  & = & p_{hit} (.9) + (1 - p_{hit}) \cdot (0.3) + 0.245 \\
  & = & .545 + 0.6 p_{hit}  
\end{eqnarray*}

Throughput, $X$, is bounded by the following two asymptotes:
$X \leq \min\left( \frac{N}{D + \E{Z}}, \frac{1}{D_{max}} \right). $

Substituting in the expressions for $D$, $\E{Z}$, and $D_{max}$ that we have already derived, as well as $N= 72$, we have:

$$X \leq \min\left( \frac{72}{.545 + 0.6 p_{hit} +  0.65 + 100 p_{miss} }, \frac{1}{0.9 p_{hit}} \right). $$

Putting this all in terms of $p_{hit}$ and removing insignificant terms, we have:

\begin{eqnarray}
X &\leq & \min\left( \frac{72}{101 - 99 p_{hit} }, \frac{11}{ p_{hit}} \right).  \label{eqn:X}
\end{eqnarray}
  
IMPORTANTLY:  Notice that the first term in (\ref{eqn:X}) is {\em increasing} in $p_{hit}$, while the second term is {\em decreasing} in $p_{hit}$.

To understand which term is more important, we need to look at
$$N^* = \frac{D + \E{Z}}{D_{max}}$$
and understand the relationship of $N = 72$ to $N^*$.

Substituting in the expressions for $D$, $\E{Z}$, and $D_{max}$ that we have already derived, we have:

\begin{eqnarray}
  N^* & =&  \frac{D + \E{Z}}{D_{max}} \nonumber \\
  & \approx & \frac{.545 + 0.6p_{hit} + 0.65 + 100 (1 - p_{hit})}{0.9 p_{hit}}  \nonumber \\
  & \approx & \frac{101 - 99 p_{hit}}{0.9 p_{hit}} \nonumber \\
  & \approx & \frac{112}{p_{hit}} - 110  \label{eqn:N*}
\end{eqnarray}

Thus $N^*$ itself also depends on $p_{hit}$.

To make sense of this, it helps to consider some values of $p_{hit}$.
\begin{itemize}
\item If $p_{hit} \leq 0.6  \Longrightarrow N^* \geq 77 > 72$.   In this case, the first asymptote dominates, which points to wanting to {\em increase} $p_{hit}$.
  \item If $p_{hit} \geq 0.7 \Longrightarrow N^* < 50 < 72$.  In this case, the second asymptote dominates, which points to wanting to {\em decrease} $p_{hit}$.
  \end{itemize}

Queueing theory also allows us to study the effect of other parameters.  For example we find (not shown here) that when the disk is faster, i.e.,  $Z_{disk}$ is smaller, then $N^*$ becomes smaller and we end up wanting to {\em decrease} $p_{hit}$ over a wider range of values.
Likewise, when the disk is slower, i.e., $Z_{disk}$ is higher, then $N^*$ becomes larger and we want to {\em increase} $p_{hit}$, unless it it already very high.

\section{Simulation and Implementation Results}

The above predictions from queueing theory are in fact exactly what happens.   We see that when $p_{hit} \leq 0.6$, higher throughput is obtained by increasing $p_{hit}$, while when $p_{hit}> 0.6$, higher throughput is obtained by decreasing $p_{hit}$.

Figure~\ref{fig:simulation100} shows the results of simulating our model to provide exact throughput.  It also shows the actual implementation results, which are a very close fit to the model results.

\begin{figure}[ht]
\centerline{\psfig{file=figs/simulation100.eps,height=2.1in}}
\caption{Simulation and implementation results for the LRU cache.  At first, throughput increases as we increase $p_{hit}$.  However after the point where $p_{hit} = 0.6$, the throughput decreases as we increase $p_{hit}$.}
\label{fig:simulation100}
\end{figure}


\section{How the Results Change for FIFO Caches}

While the LRU policy is the most commonly used policy for caching, another policy which is sometimes used is FIFO.   Under FIFO, the items in the cache are kept in a FIFO queue that is never reordered.

Specifically, in the case where item $d$ is a hit, the item just stays in its current position in the queue.  In the case where item $d$ is a miss, the item at the head of the FIFO queue is popped off and item $d$ is appended to the tail of the queue.  

The big difference then in terms of the queueing model is that we no longer have the Delink Operation.  We do still have the Tail and Head operations, however.  The queueing model for the FIFO Caching system is shown in Figure~\ref{fig:FIFOcache}. 

\begin{figure}[ht]
\centerline{\psfig{file=figs/FIFOcache.eps,height=2.5in}}
\caption{Queueing model of FIFO cache.}
\label{fig:FIFOcache}
\end{figure}

It turns out that this small change in the queueing model has a huge impact.  Specifically, we will show that for the FIFO cache, one {\em always} wants to increase $p_{hit}$.

To see why, first observe that now 
$$D_{max} = D_{tail} = 0.3 \cdot p_{miss} = 0.3 - 0.3 p_{hit}.$$

Thus, increasing $p_{hit}$ will always cause a {\em decrease} in $D_{max}$, which in turn causes an increase in throughput.

Thus we no longer have the situation where the two asymptotes of throughput are going in opposite directions, because now both throughput asymptotes favor increasing $p_{hit}$.
Specifically, we have:
$$X \leq \min\left( \frac{N}{D + \E{Z}}, \frac{1}{D_{max}} \right), $$
which simplifies to:
$$X \leq \min\left( \frac{72}{0.54(1-p_{hit}) + 0.65 + 100 - 100p_{hit}}, \frac{1}{0.3 - 0.3 p_{hit}} \right). $$
Clearly both asymptotes are increasing with $p_{hit}$, so we don't see the contradictory behavior that we witnessed for LRU caches.

\section{Other analysis and results}

We have also applied this analysis to a wide range of other caching models including the FrozenHot model, the Probabilistic LRU Model (HHVM, CacheLib), and the Clock Model.  


==> ancient/todo.tex <==

% \section{Instruction}
% There are macros e.g., \\jason, \\mor that are used for comments 

\section{Status update}
Juncheng
% have finished: 
    % restructured the document

\begin{enumerate}
    \item have incorporated the Friday discussion points 
    % \item have updated the table in intro, still needs some work
    \item Monday: added the BibTeX of work from TPC 
    \item Monday: working on adding text in intro, finished reading queueing model
\end{enumerate}

Ziyue: 
\begin{enumerate}
    \item 
\end{enumerate}

Mor: 
\begin{enumerate}
    \item Saturday: I went through the whole paper, fixing things and adding notes on what we need. 
    \item Sunday: I will spend time working on the queueing sections to figure out how to best explain things. 
\end{enumerate}

\section{Discussion}
\begin{enumerate}
    \item \jason{should we just have one figure for Probabilistic LRU? Right now, we have three figures for different probabilities; I think we can pick a disk latency, e.g., 100 us, and plot three figures. Not sure if it is a good idea}
\end{enumerate}

\section{todo list}
\subsection{Result numbers and plots}
\begin{enumerate}
    \item add SLRU @Ziyue
    % \item update results with error bars @Ziyue
    % \item update plot style, e.g., larger font, remove disk latency, use linear scale y-axis @ziyue @juncheng
    \item add the frontpage figure (might be better to share the plot script for quick iterations) @ziyue 
\end{enumerate}

\subsection{Writing}
\begin{enumerate}
    \item fix the compilation issues @Juncheng @Mor
    \item clean up the macros (I am not sure which ones we would need) @Mor
    \item Finish the intro as discussed @Juncheng
    \item Add prior work @Juncheng
    \item Add system and algorithm (sec 3) @Juncheng
    \item Add implementation and results @Ziyue @Juncheng
\end{enumerate}


==> ancient/ziv.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% ZIV STUFF %%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tikz}
\usepackage{tkz-graph}
\usepackage{xifthen}

% Use these to change the scale.
\newcommand{\rankscale}{9.2}
\newcommand{\serverscale}{0.25}
\newcommand{\multistagescale}{0.6}

\usetikzlibrary{intersections, backgrounds, shapes.arrows,
  decorations.pathreplacing}

\newcommand{\xscale}{\rankscale}
\newcommand{\yscale}{\rankscale}
\newcommand{\ticksize}{3.7}
\newcommand{\axisarrowsize}{8}
\newcommand{\xarrowsize}{(\axisarrowsize/\xscale)}
\newcommand{\yarrowsize}{(\axisarrowsize/\yscale)}

\newcommand{\ifempty}[3]{\ifthenelse{\isempty{#1}}{#2}{#3}}

\newcommand{\xguide}[3][]{%
  \draw[axis] ({#2}, 0) -- ({#2}, -\ticksize/\yscale)
  node[below] {\ifempty{#1}{$#2$}{#1}\vphantom{by}};
  \draw[guide] ({#2}, 0) -- ({#2}, {#3});}
\newcommand{\yguide}[3][]{%
  \draw[axis] (0, {#3}) -- (-\ticksize/\xscale, {#3})
  node[left] {\ifempty{#1}{$#3$}{#1}};
  \draw[guide] (0, {#3}) -- ({#2}, {#3});}

\newcommand{\axes}[4]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {$0$} -- ({#1 + \xarrowsize}, 0) node[right] {#3};
  \draw[axis, ->] (0, -\ticksize/\yscale)
  node[below] {$0\vphantom{by}$} -- (0, {#2 + \yarrowsize})
  node[above] {#4};}

\newcommand{\point}[2][primary]{%
  \filldraw[#1, very thick] #2 circle (1.8mu);}

\newcommand{\jump}[4][primary]{%
  \point[#1, fill=white]{(#2, #3)}
  \point[#1]{(#2, #4)}}

\newcommand{\job}[4][]{%
  \fill[magenta!74!blue!26] (#2-0.25, #3+0.25) rectangle ++(0.5, #4);
  \ifempty{#1}{}{%
    \fill[green!60!blue!60!gray] (#2-0.25, #3+0.25) rectangle ++(0.5, #1*#4);
    \draw (#2-0.25, #3+0.25+#1*#4) -- ++(0.5, 0);}
  \draw (#2-0.25, #3+0.25) rectangle ++(0.5, #4);}

\tikzset{%
  style={font=\small},
  rank plot/.style={x=\xscale, y=\yscale, thick,
    baseline={([yshift={-\ht\strutbox}]current bounding box.north)}},
  axis/.style={thick},
  primary/.style={ultra thick, color=cyan!97!black},
  bubble/.style={ultra thick, dash pattern=on 3.5pt off 1.5pt,
    color=red!39!yellow!87!black},
  bubblefill/.style={color=red!37!yellow!45},
  guide/.style={thick, densely dotted}}

\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

